Convergence of TD(0) under Polynomial Mixing with Nonlinear Function Approximation

Temporal Difference Learning (TD(0)) is fundamental in reinforcement learning, yet its finite-sample behavior under non-i.i.d. data and nonlinear approximation remains unknown. We provide the first high-probability, finite-sample analysis of vanilla TD(0) on polynomially mixing Markov data, assuming only Holder continuity and bounded generalized gradients. This breaks with previous work, which often requires subsampling, projections, or instance-dependent step-sizes. Concretely, for mixing exponent $\beta > 1$, Holder continuity exponent $\gamma$, and step-size decay rate $\eta \in (1/2, 1]$, we show that, with high probability, \[ \| \theta_t - \theta^* \| \leq C(\beta, \gamma, \eta)\, t^{-\beta/2} + C'(\gamma, \eta)\, t^{-\eta\gamma} \] after $t = \mathcal{O}(1/\varepsilon^2)$ iterations. These bounds match the known i.i.d. rates and hold even when initialization is nonstationary. Central to our proof is a novel discrete-time coupling that bypasses geometric ergodicity, yielding the first such guarantee for nonlinear TD(0) under realistic mixing.

==> checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}.
    \item[] Justification: We clarify in the abstract, and throughout the paper, on multiple occasions.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}.
    \item[] Justification: Addressed in conclusion with four future work directions.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{}.
    \item[] Justification: All proofs and theorems have assumptions stated, and restated when proved in appendix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerNA{}.
    \item[] Justification: No experiments
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNA{}.
    \item[] Justification: no data or code
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerNA{}.
    \item[] Justification: no experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNA{}.
    \item[] Justification: no experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerNA{}.
    \item[] Justification: no experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The work is purely theoretical and does not touch on any of the topics listed in the code of ethics guideline.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{}.
    \item[] Justification: It's purely theory, there are no applications discussed.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}.
    \item[] Justification: no risks posed by our bounds.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerNA{}.
    \item[] Justification: does not use any assets
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{}.
    \item[] Justification: no assets developed
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}.
    \item[] Justification: no human subjects or crowdsourcing
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}.
    \item[] Justification: no human subjects
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{}.
    \item[] Justification: No LLM usage
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> figs_tables/comparisons.tex <==
\begin{table*}[t]
    \centering
    \renewcommand{\arraystretch}{1.2}
    \caption{Comparison of error bounds for TD(0) algorithm with linear functional approximation.}
    \setlength{\tabcolsep}{3pt} % Reduce spacing
    \resizebox{\textwidth}{!}{ % Forces table to fit text width
    \begin{tabular}{lccccccc}
        \toprule
        \textbf{Authors} & B. (\citeyear{bhandari18}) & D. (\citeyear{dalal2018finite}) & L. and S.(\citeyear{lakshminarayanan2018linear}) & P. (\citeyear{patil2023finite}) & L.(\citeyear{li2024high}) & S. (\citeyear{samsonov24}) & \textbf{This paper} \\
        \midrule
        \textbf{Algorithm type} & P-R & Last iterate & P-R & P-R & P-R & P-R & Last iterate \\
        \textbf{Step size schedule} & $1/\sqrt{t}$ & $1/k^\kappa$ & constant $\alpha$ & constant $\alpha$ & constant $\alpha$ & constant $\alpha$ & $1/t^\gamma, \gamma>\frac{1}{2}$ \\
        \textbf{Universal step size} & \cmark & \cmark & \cmark & \cmark & \xtimes & \cmark & \cmark \\
        \textbf{Markovian data} & \cmark & \xtimes & \xtimes & \cmark & \xtimes & \cmark & \cmark \\
        \textbf{High-order bounds} & \xtimes & \cmark & \xtimes & \cmark & \cmark & \cmark & \cmark \\
        \textbf{No projection} & \xtimes & \cmark & \cmark & \xtimes & \cmark & \cmark & \cmark\\
        \textbf{Mixing properties} & Geometric & \xtimes & \xtimes & Geometric & \xtimes & Geometric & Polynomial\\
        \textbf{Function} & Linear & Linear & Linear & Linear & Linear & Linear & Deep ReLU Network\\
        \textbf{No Data Dropping} & \cmark & \cmark & \cmark & \cmark & \cmark & \xtimes  & \cmark \\
        \bottomrule
    \end{tabular}
    }
    \vspace{0.5em} % Reduce unnecessary space
    \raggedright
%    \textsuperscript{(1)} (Bhandari et al., 2018) considers constant step size $\alpha = 1/\sqrt{n}$ with $n$ being total number of iterations and provides suboptimal MSE bound of order $\tilde{\mathcal{O}}(1/\sqrt{n})$;
%    \textsuperscript{(2)} (Dalal et al., 2018) uses last iterate and decreasing step size schedule with $\alpha_k = 1/k^\kappa$. Hence, the corresponding bias forgetting rate is sublinear, and the $n$-step MSE is of order $\tilde{\mathcal{O}}(1/n^\kappa)$;
%    \textsuperscript{(3)} (Patil et al., 2023) uses projections to prove the concentration bounds, and the definition of the projection set involves the unknown parameter $\theta_*$. 
\end{table*}

==> old/12_deep_relu_parm_convergence.tex <==
\subsection{Auxiliary Lemmas for Deep ReLU Networks}
\label{sec:aux-lemmas-relu}

We work under Assumptions: bounded rewards $(|R_t|\le R_{\max})$, \(\beta\)-polynomial mixing $(\beta>1)$, and a polynomially decaying step size \(\alpha_t=c\,t^{-\eta}\) with $\tfrac12<\eta<1$.  Throughout, each layer-weight matrix satisfies \(\|W_\ell\|_2\le B\) and inputs obey $\|X_t\|_2\le X_{\max}$.

\paragraph{Notation.}  Let $n$ denote network depth and $d$ the total number of parameters.  For any $x$, the TD sub‑gradient is
\[
  g_t(\theta)
  \;=\;
  \bigl(R_t+\gamma V_{\theta}(X_{t+1})-V_{\theta}(X_t)\bigr)
  \,\nabla_{\!\theta} V_{\theta}(X_t).
\]

\begin{lemma}[Uniform Gradient Bound]\label{lem:uniform-grad}
For every $\theta$ with $\|W_\ell\|_2\le B$ and every $x$,
\[
  \|\nabla_{\!\theta}V_{\theta}(x)\|_F\;\le\;G,
  \qquad
  G\;:=\;n B^{\,n}\bigl(X_{\max}+1\bigr).
\]
\end{lemma}
\begin{proof}
Inside any fixed activation region the network can be written $V_\theta(x)=A_\theta x$ with
$A_\theta=\prod_{j=1}^n W_jD_j$, where diagonal gate matrices $D_j$ satisfy $\|D_j\|_2\le1$.  Taking a single layer $W_\ell$ we have
\[
  \frac{\partial V_\theta(x)}{\partial W_\ell}
   =\bigl(\prod_{j>\ell}W_jD_j\bigr)\,D_\ell\bigl(\prod_{j<\ell}D_jW_j\bigr)x.
\]
Applying the Frobenius–spectral inequality and $\|D_j\|_2\le1$ yields
$\bigl\|\tfrac{\partial V}{\partial W_\ell}\bigr\|_F\le B^{n-1}X_{\max}$.  Summing over $\ell=1,\dots,n$ and allowing an additive bias term (size at most~$1$) gives the claimed constant $G$.
\end{proof}

\begin{lemma}[Finite Region Crossings]\label{lem:finite-regions}
Let $\gamma_{\min}>0$ denote the minimum distance in parameter space between two adjacent activation regions—that is, the smallest step size needed to change the activation pattern at any layer. Under weight-boundedness $\|W_\ell\|_2\le B$ and finite input norm $\|X_t\|_2\le X_{\max}$, there exists such a constant depending only on $(B, X_{\max}, n)$. A single TD(0) update satisfies $\theta_{t+1}-\theta_t = -\alpha_t g_t$, so
\[
  \kappa_t\;\le\;\frac{\|g_t\|\,\alpha_t}{\gamma_{\min}}\;\le\;\frac{G^2\,\alpha_t}{\gamma_{\min}}.
\]
Because $\sum_t\alpha_t<\infty$ for $\eta>\tfrac12$, we have $\sum_t\kappa_t<\infty$ almost surely, so the iterate path crosses only finitely many activation regions.
\end{lemma}

\begin{proof}
For a ReLU network, each unit's pre-activation induces a hyperplane in parameter space where its activation switches on/off. These hyperplanes correspond to the zero level sets of affine functions of the weights:
\[
  \theta \;\mapsto\; \langle w_{i,\ell}, h_{\ell-1}(x; \theta) \rangle
\]
where $w_{i,\ell}$ is the $i$‑th row of the layer $\ell$ weight matrix and $h_{\ell-1}$ is the previous layer’s output. The set of points in $\theta$‑space where this scalar product equals zero defines an activation boundary.

Since $x$ is bounded and $\|W_\ell\|_2\le B$, each such hyperplane has bounded curvature and bounded normal vector length. This ensures the distance between two adjacent activation regions (with different binary patterns) is lower bounded by a positive $\gamma_{\min} > 0$. This is a direct consequence of Lemma 1 in Arora et al. (2018), which bounds the number of linear regions in deep ReLU networks and implies piecewise-linear partitions are well-separated under bounded weights.

Now, each update $\theta_{t+1}-\theta_t = -\alpha_t g_t$ moves by at most $\|g_t\|\,\alpha_t\le G^2 \alpha_t$. Thus, the number of activation region boundaries that can be crossed at time $t$ is at most
\[
  \kappa_t \;\le\; \frac{\|\theta_{t+1}-\theta_t\|}{\gamma_{\min}} \;\le\; \frac{G^2 \alpha_t}{\gamma_{\min}}.
\]
Since $\sum_t \alpha_t < \infty$, it follows that $\sum_t \kappa_t < \infty$, and the total number of distinct activation region transitions is finite almost surely.
\end{proof}

\begin{lemma}[Piecewise‑H\"older TD Gradient]\label{lem:holder}
Inside a single activation region the Jacobian $\theta\mapsto g_t(\theta)$ is affine, hence
$\|g_t(\theta)-g_t(\theta')\|\le G_1\,\|\theta-\theta'\|$ with $G_1:=2G(R_{\max}+X_{\max})$.  By Lemma~\ref{lem:finite-regions} only finitely many regions are entered, so the same Lipschitz constant works globally on the iterate set.  Define
\[
  L\;:=\;G_1\bigl(1+R_{\max}\bigr).
\]
Then $\theta\mapsto\E[g_t(\theta)]$ is $L$‑H\"older along the entire training trajectory.
\end{lemma}

\vspace{1em}
\noindent Theorem~4.3 now inherits constants $(G,L)$ explicitly.

\subsection{Proof of Theorem \ref{theorem:hp-nonlinear-bounds}: High‑Probability Bounds, Nonlinear Function Approximation}
\label{app:proof-hp-nonlinear}

\paragraph{Theorem \ref{theorem:hp-nonlinear-bounds} (High‑Probability Error Bounds, Deep ReLU).}
\textit{Under Assumptions~2.1–2.3 and auxiliary Lemmas~\ref{lem:uniform-grad}–\ref{lem:holder}, let $\delta\in(0,1)$.  With probability at least $1-\delta$ the TD(0) parameter error satisfies}
\[
  \|\theta_t-\theta^*\|
  \;\le\;C_\delta\,t^{-(\beta-1)/2}\;+
           C'_\delta\,t^{-\eta\beta},
\]
\textit{where}
$C_\delta:=4G\sqrt{\log(4/\delta)}$ and
$C'_\delta:=\tfrac{4L}{\lambda_{\min}(H)}$.

\begin{proof}
\paragraph{1) Error decomposition.}
Set $\Delta_t:=\theta_t-\theta^*$.  Writing the TD(0) update around the root gives
\[
  \Delta_{t+1}=(I-\alpha_t H)\Delta_t+\alpha_t(M_t+\zeta_t),
\]
with $H:=\nabla_\theta\E[g_t(\theta^*)]$ positive‑definite (Section~2.3),
$M_t:=g_t-\E[g_t\mid\mathcal F_{t-1}]$ a martingale difference, and $\zeta_t:=\E[g_t(\theta_t)]-\E[g_t(\theta^*)]$.

\paragraph{2) Martingale term $M_t$.}
Lemma~\ref{lemms:uniform error bounds} bounds $\|M_t\|\le2G^2$.  Using the Merlev\`ede–Peligrad–Rio Bernstein inequality for $\beta$‑mixing sequences,
\[
  \Pr\Bigl(\bigl\|\sum_{k=1}^t\alpha_k M_k\bigr\|\ge u\Bigr)
       \le 2d\exp\!\bigl(-\tfrac{c\,u^2}{G^4\sum_k\alpha_k^2+uG^2 t^{1-\beta}}\bigr).
\]
Choosing $u=C_\delta t^{-(\beta-1)/2}$ with $C_\delta$ above and noting $\sum_k\alpha_k^2<\infty$ yields the high‑probability martingale bound $\|\sum_{k\le t}\alpha_k M_k\|\le C_\delta t^{-(\beta-1)/2}$.

\paragraph{3) Deterministic remainder $\zeta_t$.}
By Lemma~\ref{lem:holder},
$\|\zeta_t\|\le L\,\|\Delta_t\|$.
Insert this into the recursion and invoke a discrete Gr\"onwall inequality:
\[
  \|\Delta_t\|\le e^{-\lambda_{\min}(H)\sum_{k\le t}\alpha_k}\|\Delta_0\|
               +\frac{L}{\lambda_{\min}(H)}\alpha_{t-1}.
\]
With $\alpha_{t-1}=c(t-1)^{-\eta}$ and $\sum_{k\le t}\alpha_k\ge c' t^{1-\eta}$ we obtain
$\|\Delta_t\|\le C'_\delta t^{-\eta\beta}$ as claimed.

\paragraph{4) Union bound.}  The martingale and remainder events each fail with probability at most $\delta/2$; a union bound gives overall success probability $1-\delta$.
\end{proof}

\paragraph{Remark.}  If the chain is geometrically mixing (\(\beta{\to}\infty\)) the first term improves to $O\bigl((\log t)/t^{1/2}\bigr)$.


==> sections/00_abstract.tex <==
\begin{abstract}
Temporal Difference (TD) learning is a foundational algorithm in reinforcement learning.
A core challenge is establishing its convergence properties under general, non-i.i.d. data and nonlinear function approximation. Previous work has proven convergence of TD(0) in the asymptotic regime or under strong assumptions such as geometric mixing, data dropping, or instance-dependent step sizes.
In this paper, we go a step further and analyze the high-probability, finite-sample performance of TD(0) under realistic conditions. We work directly with unmodified TD(0) using nonlinear function approximation, assuming only Hölder continuity and bounded generalized gradients. The data is generated by a Markov process with polynomial mixing, and all samples are used without subsampling or projections.
We show that TD(0) achieves an \( \varepsilon \)-accurate estimate of the value function w.h.p. after \( \mathcal{O}(1/\varepsilon^2) \) iterations, up to problem-dependent constants involving the mixing rate and step size decay.
These bounds match the known i.i.d. rates and hold even when initialization is nonstationary.
We introduce a novel discrete-time coupling analysis that yields high-probability convergence bounds for TD(0) with nonlinear function approximation under polynomial mixing, without any need for data dropping, projections, or geometric ergodicity. Our result is, to our knowledge, the first high-probability convergence guarantee for TD(0) under polynomial mixing and nonlinear approximation, without algorithmic modification or step-size tuning.
\end{abstract}


==> sections/10_conclusion.tex <==
\section{Conclusion}

In this work, we provided a rigorous analysis of the stability and convergence properties of the Temporal Difference (TD(0)) learning algorithm for linear and non-linear under polynomial mixing for markov processes. By coupling arguments, we demonstrate that the mixing properties of the Markov process can be leveraged to achieve meaningful high-probability bounds, even without assuming strong smoothness or exponential stability.

Furthermore, our analysis shows that polynomial mixing conditions suffice to ensure robust convergence, broadening the applicability of TD learning to a wider range of reinforcement learning problems. This relaxation of assumptions opens the door to studying TD learning in more realistic and challenging settings where strong regularity conditions are impractical.

Future work may focus on:
\begin{enumerate}
    \item Impact of weaker mixing conditions, such as sub-polynomial mixing, on convergence rates.
    \item Remove the need for H\"older continuous functions
    \item Dynamically adjust step sizes based on the observed mixing properties.
    \item Extend to Deep Neural Networks
\end{enumerate}

We hope these insights lead to more general and robust reinforcement learning methods.
